Search for Prompt Production of $\chi_{c}$ and X(3872) in e^+e^- Annihilations

We have searched for prompt production of $\chi_{c1}$, $\chi_{c2}$ and X(3872) in continuum e^+e^- annihilations using a 386 fb^{-1} data sample collected around $\sqrt{s} = 10.6$ GeV with the BABAR detector using the $\gamma J/\psi$ decay mode. After accounting for the feed-down from $\psi(2S)\to\gamma\chi_{c1,2}$, no significant signal for prompt $\chi_{c1,2}$ production is observed. We present improved upper limits on the cross-section, with the rest of the event consisting of more than two charged tracks, to be 77 fb for $\chi_{c1}$ and 79 fb for $\chi_{c2}$ with $e^+e^-$ center-of-mass frame $\chi_c$ momentum greater than 2.0 GeV at 90% confidence level. These limits are consistent with NRQCD predictions. We also set an upper limit on the prompt production of X(3872) through the decay $X(3872)\to \gamma J/\psi$.

==> abstract.tex <==
\begin{abstract}
  We have searched for prompt production of $\chi_{c1}$, $\chi_{c2}$ and $X(3872)$
  in continuum $e^+e^-$ annihilations using a 386 fb$^{-1}$ data sample
  collected around $\sqrt{s} = 10.6$ GeV with the $BABAR$ detector
  using the $\gamma J/\psi$ decay mode.
  After accounting for the feed-down from $\psi(2S)\rightarrow\gamma\chi_{c1,2}$,
  no significant signal for prompt $\chi_{c1,2}$ production is observed. We
  present improved upper limits on the cross-section,   
  with the rest of the event consisting of more than two charged tracks, to be 
  77 fb for $\chi_{c1}$ and 79 fb for $\chi_{c2}$
  with $e^+e^-$ center-of-mass frame $\chi_c$ momentum greater than 2.0 GeV
  at 90\% confidence level.
  These limits are consistent with NRQCD predictions.  
  We also set an upper limit on the prompt production of $X(3872)$ through the decay
  $X(3872)\rightarrow \gamma J/\psi$. 
\end{abstract}

